An Information-Theoretic Approach to Transferability in Task Transfer Learning

Task transfer learning is a popular technique in image processing applications that uses pre-trained models to reduce the supervision cost of related tasks. An important question is to determine task transferability, i.e. given a common input domain, estimating to what extent representations learned from a source task can help in learning a target task. Typically, transferability is either measured experimentally or inferred through task relatedness, which is often defined without a clear operational meaning. In this paper, we present a novel metric, H-score, an easily-computable evaluation function that estimates the performance of transferred representations from one task to another in classification problems using statistical and information theoretic principles. Experiments on real image data show that our metric is not only consistent with the empirical transferability measurement, but also useful to practitioners in applications such as source model selection and task transfer curriculum learning.

==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we validate and analyze our transferability metric through  experiments on real image data. \footnote{Test data and code can be found at  \href{https://github.com/YaojieBao/An-Information-theoretic-Metric-of-Transferability}{https://goo.gl/uoXj8m
} } The tasks considered cover both object classification and  non-classification tasks in computer vision, such as depth estimation and 3D (occlusion) edge detection.  
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Validation of transfer performance}
 
To demonstrate that our transferability metric is indeed a suitable measurement for task transfer performance, we compare it with the empirical performance of transfering features learned from  ImageNet $1000$-class  classification  (\cite{imagenet})  to  Cifar $100$-class classification  (\cite{cifar}), using a network similar to Figure~\ref{fig:tl-network}.  Comparing to ImageNet-1000, Cifar-100 has smaller sample size and its images have lower resolution. Therefore it is considered to be a more challenging task than ImageNet, making it a suitable case for transfer learning. In addition,  we use a pretrained ResNet-$50$ as the source model due to its high performance and regular structure.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Source task selection.}
The training data for the target task in this experiemnt consists of  $20,000$  images randomly sampled from Cifar-$100$. It is further split 9:1 into a training set and a testing set. The transfer network was trained using stochastic gradient descent with batch size $20,000$ for 100 epochs.
Figure~\ref{fig:cifar}.a compares the H-score of transferring from five different layers (4a-4f) in the source network   with the target log-loss and test accuracy of the respective features. As H-score increases,  log-loss of the target network decreases almost linearly while the training and testing accuracy increase. Such behavior is consistent with our expectation that H-score reflects the learning performance of the target task. We also demonstrated that target sample size does not affect the relationship between H-score and log-loss (Figure~\ref{fig:cifar}.b). 
This experiment also showed another potential application of H-score for selecting the most suitable layer for fine-tuning in transfer learning. In the example, transfer performance is better when an upper layer of the source networks is transferred. This could be because the target task and the source task are  inherently similar such that the representation learned for one task can still be discriminative for the other.  
\begin{figure}[htp]
\centering
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{cc }
\includegraphics[height=0.12\textheight]{results/h-score_performance.png} &
\includegraphics[height=0.12\textheight]{images/cifar100-samplesize-crop.pdf} \\
(a) & (b) \\
\includegraphics[height=0.12\textheight]{results/acc_vs_transfer.png} &  \includegraphics[height=0.12\textheight]{images/acenn.pdf}\\
(c) & (d)  
\end{tabular}
\caption{\label{fig:cifar}H-score and transferability vs. the empirical transfer performance measured by log-loss, training and testing accuracy. a.) Performance of ImageNet-1000 features from layers 4a-4f for Cifar-100 classification.   b.)  Effect of sample size (5K-50K) on H-score for Cifar 100. d.) Architecture for the neural network implementation of the soft HGR problem } %  c.): Transferability from ImageNet-1000 to 4 different target tasks based on Cifar-100.  }
\label{fig:logloss}
\end{figure}   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\noindent\bf Validation of Transferability.}  We further tested our transferability metric for selecting the best target task for a given source task. In particular, we constructed 4 target classification tasks with 3, 5, 10, and 20 object categories from the Cifar-100 dataset.  We then computed the transferability from ImageNet-1000 (using the feature representation of layer 4f) to the target tasks. The results are compared to the empirical transfer performance trained with batch size 64 for 50 epochs in Figure\ref{fig:logloss}.c. We observe a similar behavior as the H-score in the case of a single target task in Figure~\ref{fig:logloss}.a, showing that transferability can directly predict the  empirical transfer performance.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Task transfer for 3D scene understanding}  
In this experiment, we solve the source task selection problem for  a  collection of 3D scene-understanding tasks using the Taskonomy dataset from  \cite{zamir2018taskonomy}.  In the following, we will introduce the experiment setting and explain how we adapt the transferability metric to pixel-to-pixel recognition tasks.  Then we compare transferability with  {\em task affinity}, an empirical transferability metric proposed by \cite{zamir2018taskonomy}.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\noindent\bf Data and Tasks. }  
The Taskonomy dataset contains 4,000,000 images of indoor scenes of 600 buildings. Every image has annotations for $26$ computer vision tasks. We randomly sampled $20,000$ images  as training data. Eight tasks were chosen for this experiment, covering both classifications and lower-level pixel-to-pixel tasks. Table~\ref{tab:tasks}  summaries the specifications of these tasks. %Detailed description of these tasks can be found in \cite{zamir2018taskonomy}.
%\begin{figure}[ht]
%\centering
%\includegraphics[width=0.35\textwidth]{results/tasks.png}
%\caption{\label{fig:tasks}  Ground truth of different tasks for a given query image.}
%\end{figure}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\noindent\bf Feature Extraction and Data Preprocessing. }\label{sssec:preprocess} 
For each task, \cite{zamir2018taskonomy} trained a fully supervised network with an encoder-decoder structure. When testing the transfer performance from   $\mathcal{T}_S$ to   $\mathcal{T}_T$, the encoder output of $\mathcal{T}_S$ is used for training the decoder of $\mathcal{T}_T$. % (Figure~\ref{fig:encode-decode}). 
For a fair comparison, we use the same trained encoders to extract source features. The output dimension of all encoders are   $16 \times 16 \times 8$ and we flatten the output into a vector of length $2048$. To reduce the computational complexity, we also resize the ground truth  images into $64\times 64$. 

For classification tasks, H-score can be easily calculated given the source features. But for pixel-to-pixel tasks such as Edges and Depth, their ground truths are represented as images, which can not be quantized easily. 
As a workaround,  we cluster the pixel values in the ground truth images into a palette of $16$ colors. Then compute the H-score of the source features with respect to each pixel, before aggregating them into a final score by averaging over the whole image.  
 
We ran the experiment on a workstation with  $3.40$ GHz $\times 8$ CPU and $16$ GB memory. Each pairwise H-score computation finished in less than one hour including preprocessing. 
Then we rank the source tasks according to their H-scores of a given target task and compare the ranking with that in \cite{zamir2018taskonomy}. 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[h!]
\centering 
% \begin{minipage}[c]{0.32\textwidth}
%\centering
%  \scalebox{0.7}[0.7]{
%  \begin{tabular}{p{1.9cm}llp{1cm}}
%    \toprule
%	Tasks & $k$ & Output & Quantize -level\\
%    \midrule
%    2D Edges & 2048 & images & 16 \\
%    3D Occlusion Edges & 2048 & images & 16 \\
%    2D Keypoints & 2048 & images & 16 \\
%   3D Keypoints & 2048 & images & 16 \\
%    Reshading & 2048 & images & 16 \\
%    Depth & 2048 & images & 16 \\
%    \midrule
%    Object Class. & 2048 & labels & none \\
%   Scene Class. & 2048 & labels & none \\
%    \bottomrule
%  \end{tabular}
%  }
%  \caption{\label{tab:tasks}Task descriptions}
%  \end{minipage} 
\begin{minipage}[c]{0.67\textwidth}
\includegraphics[width=1\textwidth]{results/order1ranking2.pdf}
\caption{\label{fig:tasko-hscore} Ranking comparison between transferability and affinity score. }
\end{minipage} 
\end{figure*}

{\noindent\bf Pairwise Transfer Results. } 
Source task ranking results using transferability and affinity are visualized side by side in Figure~\ref{fig:tasko-hscore}, with columns representing source tasks and rows representing target tasks. 
For classification tasks (the bottom two rows in the transferability matrix), the top two transferable source tasks are identical for both methods. The best source task is the target task itself, as the encoder is trained on a task-specific network with much larger sample size. Scene Class. and Object Class. are ranked second for each other, as they are semantically related. Similar observations can be found in 2D pixel-to-pixel tasks (top two rows). The results on lower rankings  are  noisier.
 
A slightly larger difference between the two rankings can be found in 3D pixel-to-pixel tasks, especially 3D Occlusion Edges and 3D Keypoints. Though the top four ranked tasks of both methods are exactly the four 3D tasks. It could indicate that these low level vision tasks are closely related to each other so that the transferability among them are inherently ambiguous.  We also computed the ranking correlations between transferability and affinity using Spearman's R and Discounted Cumulative Gain (DCG). Both criterion show positive correlations for all target tasks. The correlation is especially strong with DCG as  higher ranking entities are given larger weights.
%Never the less, the The top 3 source tasks to Image Reshading and 3D edges for both methods are also the same except for slightly different orders. For some target tasks, however, our results differ from task affinity. One such example is 3D Keypoints, where Reshading is ranked first in our method but only the fourth in task affinity. 

The above observations inspire us to define a notion of task relatedness, as some tasks are frequently  ranked high  for each other. Specifically, we represent each task with a vector   consisting of H-scores of all the source tasks, then apply agglomerative clustering over the task vectors. As shown in the dendrogram in Figure~\ref{fig:tasko-hscore}, 2D tasks and most 3D tasks are grouped into different clusters, but on a higher level, all pixel-to-pixel tasks are considered one category compared to the classifications tasks. 

\begin{figure*}[h!]
\begin{minipage}[b]{0.63\textwidth}
\centering
 \includegraphics[width=1\textwidth]{results/order2all.pdf}
 \caption{\label{fig:order2ranking}Ranking of second order transferability for all recognition tasks}
\end{minipage}
\hfill
\begin{minipage}[b]{0.35\textwidth}
\centering
\includegraphics[width=1\textwidth]{results/order22.png}
\caption{First and second order pixel-wise transferability to Depth.}
\label{fig:order2}
\end{minipage}
\end{figure*}
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\noindent\bf Higher Order Transfer.}  
Sometimes we need to combine features from two or more source tasks for better transfer performance. A common way to combine features  from multiple models in deep neural networks is feature concatenation.  For such problems, our transferability definition can be easily adapted to high order feature transfer,  by computing the H-score of the concatenated features. 
 Figure~\ref{fig:order2ranking} shows the ranking results of all combinations of source task pairs for each target task. For all tasks except for 3D Occlusion Edges and Depth,  the best seond-order source feature is the combination of the top two  tasks of the first-order ranking. We examine the exception in Figure ~\ref{fig:order2}, by visualizing the pixel-by-pixel H-scores of first and second order transfers to Depth using a heatmap (lighter color implies a higher H-score). Note that different source tasks can be good at predicting different parts of the image.   The top row shows the results of combining tasks with two different ``transferability patterns" while the bottom row shows those with similar patterns. Combining tasks with different transferability patterns has a more significant improvement to the overall performance of the target task. 
 %As can be seen, different source tasks can be good at predicting different parts of the image. Here arises a natural question : can we combine the source tasks according to the heat map to improve the overall transfer performance. Experiments tell us Yes.  Another interesting observation appears when we look at the heat map of H-scores for a target task like Depth. As can be seen, different source tasks can be good at predicting different parts of the image. Here arises a natural question : can we combine the source tasks according to the heat map to improve the overall transfer performance. Experiments tell us Yes. %The calculation of transferability keeps the same except that the dimension of features becomes twice as original. 
%The results are shown in Figure (\ref{fig:order2}). The target task is Depth. Each image corresponds to a transfer with source tasks marked below. The first row shows the results of combining tasks with different 'strengths' while the last one shows those with the same 'strengths'.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Transferability for efficient transfer policy}
In this experiment, we show how to develop efficient transfer policy for tag prediction based on pairwise transferability using NUS-WIDE dataset from[].

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\noindent\bf Data and Tasks. }  The NUS-WIDE dataset contain 161,789 web images for training and 107,859 images for evaluation. Its tag set consists of 81 concepts, among which we select 36 common concepts without any ambiguity. The selected concepts are 'beach', 'birds', 'boats', 'bridge', 'buildings', 'cars', 'cat', 'clouds', 'dancing', 'dog', 'fish', 'flowers', 'garden', 'grass', 'house', 'lake', 'leaf', 'moon', 'mountain', 'ocean', 'person', 'plants', 'rainbow', 'rocks', 'running', 'sand', 'sky', 'sports', 'street', 'sun', 'swimmers', 'town', 'tree', 'vehicle', 'water', 'window'. The NUS-WIDE dataset provides six types of low-level features. In this experiment, we use the 500-D bag of words feature based on SIFT descriptions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\noindent\bf Feature Extraction and Data Preprocessing. } For each concept whose prediction is considered as an unbalanced binary classification task, we train a 4-layer fully-connected neural network with batch-size being 2048 for 50 epochs. For an arbitrary target task, the layer 3  dropout output of the source tasks is used to calculate the H-scores.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\noindent\bf Developing transfer policy. } 
We create an undirected graph with each task as a node and H-scores as the edge weight, then we find the minimum spanning tree and indicate the transfer direction. The result is shown in Figure\ref{fig:minspantree}. Most of the transfer policies are in line with human perception. For example,  the feature for predicting 'people' is useful for predicting 'dancing'; the feature for predicting 'cars' is useful for predicting 'street'; the feature for predicting 'clouds' is useful for predicting 'sky'.   

\begin{figure*}[h!]
\begin{minipage}[c]{0.20\textwidth}
\centering 
\includegraphics[width=1\textwidth]{mst-taskonomy.pdf} 
\caption{\label{fig:nn} NN. }
\end{minipage} 
\hfill
\begin{minipage}[c]{0.800\textwidth}
\centering 
\includegraphics[width=1\textwidth]{graph5.png}
\caption{\label{fig:minspantree} Minimum spanning tree. }
\end{minipage} 
\end{figure*}




==> hscore-old.tex <==
\subsection{H-Score}
%In this section, we present a performance metric of a given feature representation for a learning task.  %Then we give the operational meaning of this metric from the information geometry view.

%In this section we introduce H-score, a measurement for the effectiveness of features in learning tasks. 
 
%Consider a classification task of inferring the joint probability $P_{YX}$ from paired observations of the input variable $X$ and label $Y$. 
For a classification task involving input variable $X$ and label $Y$, most learning algorithms work by finding a $k$-dimensional functional representation $f(x)$ of $X$ that is most discriminative for the classification. %{\color{red}For example, in a deep neural network with cross-entropy loss, the network learns through backpropagation  an activation function $f$ which is fed into a softmax output layer.} % We assume $f(x)$ is zero-mean, which can be achieved by $f(x) := f(x)-\E[f(x)]$ 
To measure how  effective $f(x)$ is in predicting $Y$, rather than train the model via gradient descent and evaluate its accuracy, we present an analytical approach based on the definition below:
% let $f(X)$ be an aribitrary zero-mean feature function of $X$. We define a performance measurement for the as

\begin{definition}\label{def:hscore} Given data matrix $X\in \R^{m\times d}$ and label $Y\in \{1,\dots,|\Y|\}$. Let $f(x)$  be a $k$-dimensional, zero-mean feature function. The H-Score of $f(x)$ with respect to the learning task represented by $P_{YX}$  is: 
\[
\H(f) =   \textup{tr}(\cov(f(X))^{-1}\cov( \E_{P_{X|Y}}[f(X)|Y])) %||\tilde{B}\Xi (\Xi^\mathrm{T}\Xi)^{-\frac{1}{2}} ||_F^2 ,\quad \text{ where~  }  \Xi = [\sqrt{P_X(X)}]\f(X) 
\]
\end{definition}
This definition is intuitive from a nearest neighbor search perspective. i.e. a high H-score implies  the  inter-class variance $\cov(\E_{P_{X|Y}}[f(X)|Y])$ of $f$ is large, while feature redundancy $\tr(\cov(f(X)))$ is small.  Such a feature   is discriminative and efficient for learning label Y.  More importantly,  $\H(f) $ has a deeper operational meaning related to the asymptotic error probability for a decision rule  based on $f$ in the hypothesis testing context,  discussed in the next section. %with   feature function $f(x)$, 

\subsection{Operational Meaning of H-Score} 
%In classification tasks, the H-score of a feature $f(x)$ is closely related to the asymptotic error probability of log loss.   
Without loss of generality,  we consider the binary classification task as a hypothesis testing problem: determine whether i.i.d. samples $\x^m=\{x^{(i)}\}_{i=1}^{m}$  are drawn from   distribution   $P_1=P( X|Y=0)$ or distribution $ P_2=P(X|Y=1)$. %, where $P_1,P_2$ belong to an $\epsilon$-neighborhood  $\mathcal{N}_{\epsilon}(P_0) \triangleq \{ P | \sum_{x \in \mathcal{X}}\frac{(P(x)-P_0(x))^{2}}{P_0(x)} \leq \epsilon^{2}\} $    centered at a reference distributon $P_0$.
%And denote   $\phi_i=\frac{P_i(x)-P_0(x)}{\epsilon\sqrt{P_0(x)}} $  as the {\em information vector} corresponding to $P_i$ for $i=1,2$.

   %Given $k$ normalized feature functions $f(x) = [f_1(x), \dots, f_k(x)]$, let  $\Xi(x)=[\xi_1(x),\dots,\xi_k(x)]$ be the matrix of {\em feature vectors} $\xi_i(x) = \sqrt{P_0(x)}f_i(x)$. 
   Given  k-dimensional feature $f = [f_1(x), \dots, f_k(x)]$ defined on $\x^m$ , denote the k-dimensional statistics $l(\x^m)=\frac{1}{m}\sum_{i=1}^m (f(x^{(i)}))$ for the binary hypothesis testing problem. Let $E_f$ be the error exponent of decision region $\{\x^m~|~l(\x^m)>T\}$ for $T\geq 0$, which characterizes the asymptotic error probability $P_e$ of  $l$ (i.e. $\lim_{m\rightarrow \infty} -\frac{1}{m} \log(P_e) = E^k_f$ ). %$E_f$ can be written as the squared length of a projection:  %length to the space defined by $\phi_1-\phi_2$:
%\begin{equation}\label{eq:Ehk1}
%E^k_{f} =\sum_{i=1}^k E_{f_i} = \sum_{i=l}^k \frac{\epsilon^2}{8}\left \langle \xi_i, \phi _1-\phi_2 \right \rangle ^{2} + o(\epsilon ^{2})
%\end{equation} 
 When $f(x) = \log\frac{P_1(x)}{P_2(x)}$ is the log likelihood ratio, $l$ is the minimum sufficient statistics that achieves the largest error exponent $E_f^k=\sum_{i=1}^k\frac{\epsilon^2}{8}||\phi_1-\phi_2||^2+o(\epsilon^2)$ by the Chernoff theorem. 
(See Appendix~\ref{app:errorExpo} for details.) In the rest of this paper, we assume $\epsilon$ is small.  %drop the $o(\epsilon^2)$ term .
%%

%Without loss of generality,  we consider the binary classification task as a hypothesis testing problem defined in  Section 2.1, with $P_1=P_{X|Y=0}$, and $P_2=P_{X|Y=1}$. 
For any k-dimensional feature representation $f(x)$, we can quantify its performance with respect to the learning task using its error exponent $E_f^k$. 

\begin{thm}\label{thm:errexpokD}
 Given $P_{X|Y=0}, P_{X|Y=1} \in \mathcal{N}_{\epsilon}^{\mathcal{X}}(P_{0,X})$ and features $f$ such that $\E \left[ f(X)\right]=0$ and    $\E [f(X)f(X)^\mathrm{T}]= I$, there exists some constant $c$ independent of $f$ such that  $E_f^{k}=c\mathcal{H}(f)$.  
\end{thm}
See  Appendix~\ref{app:thm1} for the proof. 
The above theorem shows that H-score $\H(f )$ is proportional to the error exponent of the decision region based on $f(x)$ when $f(x)$ is zero-mean with identity covariance.  To compute the H-score of arbitrary $f$,  we can center the features $f_S(x)-\E[f_S(x)]$, and incorporate normalization into the computation of the error exponent, which results in   Definition \ref{def:hscore}. The details are presented in Appendix~\ref{app:hscoreFull}.  %as follows:
%\begin{equation} \label{eq:BPP}  E_f^k =c || \tilde{B} \Xi (\Xi^\mathrm{T}\Xi)^{-\frac{1}{2}} ||_F^2  
%\end{equation}
%Thus we have shown that H-score $\H(f )$ is proportional to the error exponent of the decision function based on $f(x)$. 

The proof for Theorem~\ref{thm:errexpokD} uses the fact that $\mathcal{H}(f)=\|\tilde{B}\Xi\|_{F}^{2}$ , where $\tilde{B}$ is the DTM matrix, $\Xi\triangleq \left [ \xi_{1} \cdots \xi_{k} \right ]$ is the matrix composed of information vectors $\xi_{i}$  and $c$ is a constant. This allows us to infer an upper bound for the  H-score of a given learning task: 
\begin{coro}\label{co:Eh} For all normalized feature   $f(x)=[f_1(x),\dots,f_k(x)]$, its H-score satisfies $\mathcal{H}(f)\leq \sum_{i=1}^{k}\sigma_i^{2}\leq k$, where $\sigma_i$ is the ith singular value of  $\tilde{B}$. %, the DTM for this task.  
\end{coro} 
The first inequality %gives the upper bound on the error exponent, which
 is achieved when $\Xi$ is composed of the right singular vectors of $\tilde{B}$, i.e. $\max_{\Xi} ||\tilde{B}\Xi||_F^2$
% $= ||\tilde{B}\Phi||_F^2 
 $= ||\tilde{B}_{T}||_F^2$. The corresponding feature functions $\mathrm{f}_{\opt}(X)$% = [ \sqrt{P_X}]^{-1}\Phi$
  is in fact the same as the universal minimum error probability features from the maximum HGR correlation problem.    The final inequality in Corollary \ref{co:Eh}  is due to the fact all singular values of $\tilde{B}$ are less than or equal to 1. 
  

==> hypothesis_testing.tex <==
\section{Operational Meaning of H-Score}
In this section, we will show that H-score characterizes the asymptotic probability of error in the hypothesis testing context. We will start with  some background on error exponents from statistics, then explain how to estimate it using  information geometry. Finally, we will show how computing H-score   is in fact estimating the error exponent of a feature function on the sample data.


\subsection{Error Exponent and Hypothesis Testing}

Consider the binary hypothesis testing  problem over $m$ i.i.d. sampled observations $\{x^{(i)}\}_{i=1}^{m}\triangleq x^{m}$ with the following hypotheses:
$H_0: x^m \sim P_1$  or   $H_1: x^m \sim P_2$. 

 Let $P_{x^m}$ be the empirical distribution of the samples. The optimal test, i.e., the log likelihood ratio test $\log(T)=\log\frac{P_{1}(x^{m})}{P_{2}(x^{m})}$ can be stated in terms of information-theoretic quantities as follows:
%\[\log \frac{P_{1}(x^{m})}{P_{2}(x^{m})} =
\[m[D(P_{x^{m}}||P_{2}) -D(P_{x^{m}}||P_{1})]\underset{H_{1}}{\overset{H_{0}}{\gtrless}}\log T \]
where $D$ is the Kullback-Leibler (KL) divergence operator.
%The type I error of a statistic test refers to  rejecting a null hypothesis $H_0$ (false positive) and the type II error refers to   accepting the other hypothesis $H_1$ (false n. % as shown by the red and blue areas in Figure~\ref{fig:ht}.
  
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
  no markers, domain=-6:5, samples=100,
  axis lines=none,
  every axis y label/.style={at=(current axis.above origin),anchor=south},
  every axis x label/.style={at=(current axis.right of origin),anchor=west},
  height=5cm, width=10cm,
  xtick=\empty, ytick=\empty,
  enlargelimits=false, clip=false, axis on top,
  grid = major
  ]

  \addplot [fill=cyan!20, draw=none, domain=-6:0.2] {gauss(1,1)} \closedcycle;
  \addplot [fill=red!20, draw=none, domain=0.2:5] {gauss(-2,1)} \closedcycle;
  \addplot [very thick,cyan!50!black] {gauss(-2,1)};
  \addplot [very thick,cyan!50!black] {gauss(1,1)};
  
   \node [fill=none] at (axis cs:-4,0.35){$H_{0}: P_{1}$};
   \draw[->](axis cs:-3.2,0.2)--(axis cs:-4,0.3);
   \node [fill=none] at (axis cs:3,0.35){$H_{1}: P_{2}$};
   \draw[->](axis cs:2.2,0.2)--(axis cs:3,0.3);
   \node [fill=none] at (axis cs:-2,0.1){$\beta=P_{2}(A)$};
   \draw[->](axis cs:-1,0.03)--(axis cs:-2,0.07);
   \node [fill=none] at (axis cs:1.5,0.1){$\alpha=P_{1}(A^{c})$};
    \draw[->](axis cs:0.3,0.017)--(axis cs:1.5,0.07);
  \draw [dashed](axis cs:0.2,0) -- (axis cs:0.2,0.4);
  \draw[->](axis cs:0.2,0)--(axis cs:0.2,-0.1);
   \draw [latex-latex](axis cs:0.2,-0.05) -- node [fill=white] {$A$: fail to reject $H_{0}$} (axis cs:-6,-0.05);
   \draw [latex-latex](axis cs:0.2,-0.05) -- node [fill=white] {$A^{c}$:reject $H_{0}$} (axis cs:5,-0.05);
   \node [fill=white] at (axis cs:0.2,-0.15) {$P_{x^m}:D(P_{x^m}\|P_{2})-D(P_{x^m}\|P_{1})=\frac{\log T}{m}$};
\end{axis}

\end{tikzpicture}
\caption{The binary hypothesis testing problem. The blue curves shows the probility density functions for $P_1$ and $P_2$. The rejection region $A^c$ and the acceptance region $A$ are highlighted in red and blue, respectively. The vertical line indicates the decision threshold.  }
\label{fig:ht} 
\end{figure}
Further, using Sannov's theorem, we have the asymptotic probability of type \uppercase\expandafter{\romannumeral1} error:
\[ \alpha=P_{1}(A^{c}) \approx 2^{-mD(P_{1}^{*}||P_{1})} \]
where $P_{1}^{*} = \argmin _{P \in A^{c}}D(P||P_{1})$ and $A^{c}(T) = \{x^{m}: D(P_{x^{m}}||P_{2})-D(P_{x^{m}}||P_{1}) < \frac{1}{m} \log T \}$ represents the rejection region. Similarly, the asymptotic probability of  type \uppercase\expandafter{\romannumeral2} error is
\[ \beta=P_{2}(A) \approx 2^{-mD(P_{2}^{*}||P_{2})}, \]
 where $P_{2}^{*} = \argmin _{P \in A} D(P||P_{2})$ and 
 $A = \{x^{m}:$\\
  $D(P_{x^{m}}||P_{2}) -D(P_{x^{m}}||P_{1}) > \frac{1}{m} \log T \}$ represents the acceptance region (See Figure~\ref{fig:ht}). Using the Bayesian approach for hypothesis testing,    the overall error probability  of the log likelihood ratio test is defined as:
  \[ 
  P_{e}^{(m)}=\alpha P_1+\beta P_2
  \] and the {\it best achievable exponent in the Bayesian probability of error} (a.k.a. {\it error exponent}) is defined as:
\[ E = \lim_{m\rightarrow \infty}\min_{A \subseteq \mathcal{X}^{m}} -\frac{1}{m} \log P_e^{(m)}\]
 Error exponent $E$ expresses the best rate at which  the error probability decays as sample size increases for a particular hypothesis testing problem. See \cite{Cover:1991} for more background information on error exponents and its related theorems.
 
 
 
 \subsection{Estimating Error Exponents}  
 %Using concepts in local information geometry developed by \cite{makur2015efficient}, we can characterize the  error probability of using a feature of the input data to solve a learning task by a linear projection of this feature between the input and output domains. Specifically,  
   Suppose $P_1$ and $P_2$ are sampled from the $\epsilon$-neighborhood  $\mathcal{N}_{\epsilon}(P_0) \triangleq \{ P | \sum_{x \in \mathcal{X}}\frac{(P(x)-P_0(x))^{2}}{P_0(x)} \leq \epsilon^{2}\} $    centered at a reference distributon $P_0$, and let $\phi_1,\phi_2\in \R^{|\X|}$ be vectors defined as: %{\em information vector} corresponding to $P_i$ by 
   \[
   \phi_i(x)\triangleq \frac{P_i(x)-P_0(x)}{\epsilon\sqrt{P_0(x)}} 
   \]      for $i=1,2$. The following lemma express the optimal error exponent $E$  using $\phi_1$ and $\phi_2$: 

\begin{lemma}%Given zero-mean, unit variance feature function $f(x):\X\rightarrow \R$,  
Under the local assumption defined earlier, the best achievable error exponent of the binary hypothesis testing problem with probabilities $P_1$ and $P_2$ is: 
 \[  E=%D_{KL}(P_1||P_2) =
 \frac{\epsilon^2}{8}\left \| \phi _{1}-\phi_{2} \right \|^{2}+o(\epsilon^{2})\]
 where $\epsilon$ is a constant  \cite{makur2015efficient}. 
 \end{lemma}
%In the rest of this paper, we assume $\epsilon$ is small. 
 While the above lemma characterizes the asymptotic error probability distinguishing $P_1$ and $P_2$ based on the optimal decision function, most decision functions we learn from data are not optimal, as $P_1$ and $P_2$ are unknown.
Given sample data $x^m$ and an arbitrary feature function $f:\X\rightarrow\R$, which could be learned from a pre-trained model, the error exponent of the decision function based on $f$ is  reduced in a way defined by the following Lemma:%the decision function of the form  sufficient statistics $l$ whose asymptotic error probability is defined in the following lemma}: %  given samples $\x^m$ is $l =\frac{1}{m}\sum_{i=1}^m(f(x^{(i)})$. %When $f(X)$ is zero-mean and unit variance, 
%The asymptotic error probability of $l$ is defined in the following Lemma:
  
\begin{lemma}\label{lemma:mismatch}Given a zero-mean, unit variance feature function $f:\X\rightarrow \R$ and i.i.d. sampled data $x^m$, the error probability of a mismatched decision function of the form $l=\frac{1}{m}\sum_{i=1}^m (f(x^{(i)}))$ has an exponent   
\[
E_{f} = \frac{\epsilon^2}{8}\langle \xi, \phi _{1}-\phi_{2} \rangle ^{2}+o(\epsilon^{2})
\] where $\xi\in\R^{|\X|}$ is a vector with entries $\xi(x) = \sqrt{P_{0}(x)}f(x)$ \cite{makur2015efficient}.
\end{lemma} 

%Without loss of generality,  we consider the binary classification task as a hypothesis testing problem defined in  Section 2.1, with $P_1=P_{X|Y=0}$, and $P_2=P_{X|Y=1}$. For any k-dimensional feature representation $f(x)$, we can quantify its performance with respect to the learning task using its error exponent $E_f^k$.

This lemma characterizes the  error probability of using a normalized feature of the input data to solve a learning task by a linear projection of this feature between the input and output domains. Note that normalizing features to zero-mean and unit variance results in an equivalent decision function with a different threshold value, thus we can apply Lemma 2   to any features without the loss of generality. Further, it's obvious   that  the reduced   exponent $E_f$ is maximized when $\xi = \phi_1-\phi_2$, and the optimal value is exactly the optimal error exponent $E$ in Lemma 1.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%As practical learning problems mostly concern with
To estimate the reduced error exponent for multi-dimensional features,  we present the $k$-dimensional generalization of Lemma~\ref{lemma:mismatch} below: 
\begin{lemma}
\label{lemma:mismatchK}
Given $k$ normalized feature functions $f(x) = [f_1(x),\dots, f_k(x)]$, such that $\E[f_i(X)]=0$ for all $i$, and $\cov(f(X))=I$ , we define a $k$-d statistics of the form $l^{k}=(l_{1},...,l_{k})$ where $l_{i}=\frac{1}{m}\sum_{l=1}^{m}f_{i}(x^{(l)})$. Let $\xi_1,\dots,\xi_k$ be $k$ vectors  with entries  $\xi_i(x) = \sqrt{P_X(x)}f_i(x)$ , $0\leq i\leq k$. Then the error exponent of $l^k$ is
%Let  $\Xi(x)=[\xi_1(x),\dots,\xi_k(x)]$ be the corresponding {\em feature vectors} with $\xi_i(x) = \sqrt{P_X(x)}f_i(x)$. 
\begin{equation}\label{eq:Ehkd}
E^k_{f} =\sum_{i=1}^k E_{f_i} = \sum_{i=l}^k \frac{\epsilon^2}{8}\left \langle \xi_i, \phi _1-\phi_2 \right \rangle ^{2} + o(\epsilon ^{2})
\end{equation} 
\end{lemma}
\begin{comment}
\begin{proof}
According to Cram{\'e}r's theorem, the error exponent under $P_{i}$ is 

\begin{equation*}
E_{i}(\lambda) = \min _{P \in \delta(\lambda)} D(P||P_{i})
\end{equation*}
where \begin{align*}
    \delta\left(\lambda\right) \triangleq  \{P: & ~\E_{P}[f(X)^{k}]= \\
  &  \lambda\E_{P_{1}}[f(X)^{k}]+(1-\lambda)\E_{P_{2}}[f(X)^{k}] \}    
\end{align*} 
With the techniques developed in local information geometry, the above above problem is equivalent to the following problem:

\begin{equation*}
E_{i}(\lambda) = \min _{\tilde{\phi}_{\theta^{k}}\in \sigma(\lambda)} \frac{1}{2}\|\tilde{\phi}_{\theta^{k}}-\phi_{i} \|^{2}
\end{equation*}
where $\sigma(\lambda)\triangleq \left \{ \tilde{\phi}_{\theta^{k}}:\left \langle\tilde{\phi}_{\theta^{k}},\xi_{l}  \right \rangle = \left \langle \lambda\phi_{1}+(1-\lambda)\phi_{2},\xi _{l} \right \rangle, l=1,...,k \right \}$ and $i=1,2$. Further, using the equation $\tilde{\phi}_{\theta^{k}}(x)=\sum_{l=1}^{k}\theta_{l}\xi_{l}(x)+\phi_{i}(x)-\alpha(\theta^{k})\sqrt{P_{0}(x)}+o(\epsilon)$ and the equation $\alpha(\theta^{k})=o(\epsilon^{2})$, it is easy to show that $E_{1}(\lambda)=E_{1}(\lambda)$ when $\lambda=\frac{1}{2}$. Then the overall error probability has the exponent as shown in Equation (\ref{eq:Ehkd}).  
\end{proof}
\end{comment}
 The proof of this Lemma can be found in \cite{acejournal}.
  
  
%\noindent Now we are ready to derive Theorem 1.
\subsection{H-score and Error Exponents}
Now we return to the binary classification problem. Using Lemma 3, we will show the linear relationship between H-score and error exponents.
\begin{thm}\label{thm:errexpokD}
 Given $P_{X|Y=0}, P_{X|Y=1} \in \mathcal{N}_{\epsilon}^{\mathcal{X}}(P_{0,X})$ and features $f$ such that $\E \left[ f(X)\right]=0$ and    $\E [f(X)f(X)^\mathrm{T}]= I$, there exists some constant $c$ independent of $f$ such that  $E_f^{k}=c\mathcal{H}(f)$.  
\end{thm}
\begin{proof}
By Lemma \ref{lemma:mismatchK}, the L.H.S. of the equation can be written as $E_f^k =c_0 \sum_{i=l}^k \left \langle \xi_i, \phi _1-\phi_2 \right \rangle ^{2}  $ for some constant $c_0$. It follows that
\begin{align*}
c_0 &\sum_{i=l}^k \left \langle \xi_i, \phi _1-\phi_2 \right \rangle ^{2} \\
=& c_0 \left(\left(\mathrm{P}_{X|Y=0}-\mathrm{P}_{X|Y=1}\right) ^{\mathrm{T}}F\right)\left(\left( \mathrm{P}_{X|Y=0}-\mathrm{P}_{X|Y=1}\right)^{\mathrm{T}}F\right)^{\mathrm{T}}  \\
=& c_0 \left(\E[f(X)|Y=0]-\E[f(X)|Y=1]\right)^{\mathrm{T}} \cdot \\ &\left(\E[f(X)|Y=0]-\E[f(X)|Y=1]\right) \\
=& c_0 \frac{P_Y(0)+P_Y(1)}{P_Y(0)P_Y(1)}  \left(\frac{P_{Y}(0)P_{Y}(1)+P_{Y}(1)^2}{P_{Y}(0)}\right) \cdot \\ &\mathbb{E}\left[f(X)|Y=1\right]^{\mathrm{T}}\mathbb{E}\left[f(X)|Y=1\right] \\
=& c~\tr\left(\cov(\E[f(X)|Y])\right)\\
=& c~\mathcal{H}(f)
\end{align*}
The last equation uses the fact $\cov(f(X))=I$.
 \end{proof}
%  \pagebreak
   
 
  
%\changed{Given $k$ normalized feature functions $f(x) = [f_1(x),\dots, f_k(x)]$, let  $\Xi(x)=[\xi_1(x),\dots,\xi_k(x)]$ be the matrix of {\em feature vectors} $\xi_i(x) = \sqrt{P_0(x)}f_i(x)$. Given observations $\x^m$, feature $f$ is associated with a k-dimensional statistics $l(\x^m)=\frac{1}{m}\sum_{i=1}^m (f(x^{(i)}))$ for the binary hypothesis testing problem. Let $E_f$ be the error exponent of decision region $\{\x^m~|~l(\x^m)>T\}$ for $T\geq 0$, which characterizes the asymptotic error probability $P_e$ of  $l$ (i.e. $\lim_{m\rightarrow \infty} -\frac{1}{m} \log(P_e) = E^k_f$ ). $E_f$ can be written as the squared length of a projection:} %length to the space defined by $\phi_1-\phi_2$:
%\begin{equation}\label{eq:Ehk1}
%E^k_{f} =\sum_{i=1}^k E_{f_i} = \sum_{i=l}^k \frac{\epsilon^2}{8}\left \langle \xi_i, \phi _1-\phi_2 \right \rangle ^{2} + o(\epsilon ^{2})
%\end{equation} 
%\changed{When $f(x) = \log\frac{P_1(x)}{P_2(x)}$ is the log likelihood ratio, $l$ is the minimum sufficient statistics that achieves the largest error exponent $E_f^k=\sum_{i=1}^k\frac{\epsilon^2}{8}||\phi_1-\phi_2||^2+o(\epsilon^2)$ by the Chernoff theorem. 
%(See Appendix~\ref{app:errorExpo} for details.) In the rest of this paper, we assume $\epsilon$ is small.}  %drop the $o(\epsilon^2)$ term .


==> math_commands_old.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak




%%------------------------ 
 \def\X{\mathcal{X}}
 \def\x{\mathbf{x}}
 \def\Y{\mathcal{Y}}
 \def\Z{\mathcal{Z}}
 \def\H{\mathcal{H}}
 \def\N{\mathcal{N}}
 \def\cov{\textup{cov}} 
 \def\opt{\textup{opt}} 
 \def\tr{\textup{tr}}
 \def\B{\tilde{B}}
 \def\f{\textup{f}}
\newcommand{\squeze}{\vspace{-1.5mm}}
\newcommand{\squezeup}{\vspace{-2.5mm}}
\newcommand{\squeezeup}{\vspace{-3.5mm}}
\newcommand{\squeeezeup}{\vspace{-4.5mm}} 



\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
 \DeclareMathOperator*{\argmin}{arg\!\min}
 \DeclareMathOperator*{\argmax}{\arg\!\max} 
